Reclaiming Privacy and Performance over Centralized DNS

The Domain Name System (DNS) is both a key determinant of users' quality of experience (QoE) and privy to their tastes, preferences, and even the devices they own. Growing concern about user privacy and QoE has brought a number of alternative DNS services, from public DNS to encrypted and Oblivious DNS. While offering valuable features, these DNS variants are operated by a handful of providers, reinforcing a trend towards centralization that has raised concerns about privacy, competition, resilience and Web QoE. The goal of this work is to let users take advantage of third-party DNS services, without sacrificing privacy or performance. We follow Wheeler's advice, adding another level of indirection with an end-system DNS resolver, Onoma, that improves privacy, avoiding DNS-based user-reidentification by inserting and sharding requests across resolvers, and improves performance by running resolution races among resolvers and reinstating the client-resolver proximity assumption content delivery networks rely on. As our evaluation shows, while there may not be an ideal service for all clients in all places, Onoma dynamically finds the best service for any given location.

==> sections/result.tex <==
\section{Result}
\label{sec:result}
